Polynomial-Delay Enumeration of Large Maximal Matchings

Enumerating matchings is a classical problem in the field of enumeration algorithms. There are polynomial-delay enumeration algorithms for several settings, such as enumerating perfect matchings, maximal matchings, and (weighted) matchings in specific orders. In this paper, we present polynomial-delay enumeration algorithms for maximal matchings with cardinality at least given threshold $t$. Our algorithm enumerates all such matchings in $O(nm)$ delay with exponential space, where $n$ and $m$ are the number of vertices and edges of an input graph, respectively. We also present a polynomial-delay and polynomial-space enumeration algorithm for this problem. As a variant of this algorithm, we give an algorithm that enumerates all maximal matchings in non-decreasing order of its cardinality and runs in $O(nm)$ delay.

==> macro.tex <==
\newcommand{\set}[1]{\{#1\}}
\newcommand{\relmiddle}[1]{\mathrel{}\middle#1\mathrel{}}
\newcommand{\inset}[2]{\left\{#1 \relmiddle| #2\right\}}
\newcommand{\size}[1]{| #1|}
\newcommand{\order}[1]{O(#1)}

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{proposition}[lemma]{Proposition}
% \newtheorem{corollary}[lemma]{Corollary}
\newtheorem{definition}[lemma]{Definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}
% \newtheorem{problem}{Problem}
% \newenvironment{proof}{\begin{trivlist}\item[]\noindent{\bf 証明：\hspace{0.5em}}}{\qed\end{trivlist}}%\smallskip}
\newcommand{\comp}[1]{\mu(#1)}
%% macro isaac 2017

\makeatletter
\@ifpackageloaded{algorithm2e}{
\SetKwProg{Fn}{Function}{}{}
\SetKwProg{Procedure}{Procedure}{}{}
\SetKwProg{Subprocedure}{Subprocedure}{}{}
\SetKwComment{tcc}{//}{}
\SetKwFunction{Output}{Output}%
\SetKwFunction{AllChildren}{AllChildren}
\SetKwFunction{LexMin}{LexMin}
\SetKwFunction{Traverse}{Traverse}
\SetKwFunction{Traversetree}{Traverse-tree}
\SetKwInOut{AlgInput}{Input}
\SetKwInOut{AlgOutput}{Output}
\SetKwInOut{AlgPrecondition}{Pre-conditions}
\SetKwInOut{AlgInvariant}{Invariants}
}{}
\makeatother


\newcommand{\II}{I\!I\xspace}


\makeatletter
\newcommand{\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand{\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand{\problemoutput}[1]{\gdef\@problemoutput{#1}}% Store problem question
\NewEnviron{myproblem}{
  \problemtitle{}\probleminput{}\problemoutput{}% Default input is empty
  \BODY% Parse input
  \par\addvspace{.5\baselineskip}
  \noindent{
    \framebox[0.45\textwidth][c]{
        \begin{tabularx}{0.45\textwidth}{@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{{\sc \@problemtitle}} \\% Title
            \textbf{Input:}  & \@probleminput \\% Input
            \textbf{Output:} & \@problemoutput% Output
        \end{tabularx}
        }
      }
  \par\addvspace{.5\baselineskip}
}
\makeatother
